Attack-Aware Data Timestamping in Low-Power Synchronization-Free LoRaWAN

Low-power wide-area network technologies such as LoRaWAN are promising for collecting low-rate monitoring data from geographically distributed sensors, in which timestamping the sensor data is a critical system function. This paper considers a synchronization-free approach to timestamping LoRaWAN uplink data based on signal arrival time at the gateway, which well matches LoRaWAN's one-hop star topology and releases bandwidth from transmitting timestamps and synchronizing end devices' clocks at all times. However, we show that this approach is susceptible to a {\em frame delay attack} consisting of malicious frame collision and delayed replay. Real experiments show that the attack can affect the end devices in large areas up to about $50,000\,\text{m}^2$. In a broader sense, the attack threatens any system functions requiring timely deliveries of LoRaWAN frames. To address this threat, we propose a $\mathsf{LoRaTS}$ gateway design that integrates a commodity LoRaWAN gateway and a low-power software-defined radio receiver to track the inherent frequency biases of the end devices. Based on an analytic model of LoRa's chirp spread spectrum modulation, we develop signal processing algorithms to estimate the frequency biases with high accuracy beyond that achieved by LoRa's default demodulation. The accurate frequency bias tracking capability enables the detection of the attack that introduces additional frequency biases. Extensive experiments show the effectiveness of our approach.

==> 6_Design.tex <==
\subsection{Uplink Frame Arrival Timestamping}
\label{sec:design}
This section presents our approach of timestamping the uplink frame arrival by detecting the onset time of the first preamble chirp.

\subsubsection{Preliminary}
\label{subsec:preamble}

This section presents an analytic model of LoRa's CSS modulation. It is a basis for understanding the challenges of frame arrival timestamping and developing FB estimator in \sect\ref{sec:fingerprint}. A chirp is a finite-time signal with time-varying frequency that swaps the channel's bandwidth. Specifically, it can be expressed as $s(t) = A(t) \sin \left( 2\pi \int_0^t f(x) \dif x + \theta_{\mathrm{Tx}} \right)$, where $A(t)$ and $f(t)$ denote the instantaneous amplitude and frequency of the chirp at the time instant $t$, $\theta_{\mathrm{Tx}} \in [0, 2\pi)$ is the transmitter's phase that is usually unknown.

The SDR receiver generates two unit-amplitude orthogonal carriers $\sin(2\pi f_ct + \theta_{\mathrm{Rx}})$ and $\cos(2 \pi f_c t + \theta_{\mathrm{Rx}})$, where $f_c$ is the central frequency of the channel and $\theta_{\mathrm{Rx}}$ is the phase of the two self-generated carriers. After mixing the received signal with the two orthogonal carriers and applying low-pass filtering, which are standard operations of SDR, the SDR receiver yields the $I$ and $Q$ components that can be expressed as $I(t) = \frac{A(t)}{2} \cos \Theta(t)$ and $Q(t) = \frac{A(t)}{2} \sin \Theta(t)$, where the angle $\Theta(t) = 2\pi \int_0^tf(x)\dif x - 2\pi f_c t + \theta_{\mathrm{Tx}} - \theta_{\mathrm{Rx}}$. Detailed derivation is omitted here due to space limitation and can be found in \cite{lora-sync-report2}.

A LoRaWAN uplink preamble consists of eight up chirps \cite{lorawan-spec}. For a preamble chirp, $f(t) = \frac{W^{2}}{2^{S}} \cdot t - \frac{W}{2} + f_c$ for $t \in \left[ 0, \frac{2^S}{W} \right]$, where $W$ is the channel bandwidth, $S \in [6, 12]$ is the integer {\em spreading factor}, and $\frac{2^S}{W}$ is the {\em chirp time}.

The $f(t)$ increases linearly from $(f_c - W/2)$ Hz to $(f_c + W/2)$ Hz over a chirp time. The angle of the preamble chirp can be derived as $\Theta(t) = \frac{\pi W^2}{2^S} t^2 - \pi W t + \theta_{\mathrm{Tx}} - \theta_{\mathrm{Rx}}$. In this paper, we use a channel with $f_c = 869.75\,\text{MHz}$ and $W = 125\,\text{kHz}$. Fig.~\ref{fig:up-chirp} shows the $I$ data and the spectrogram of an ideal preamble chirp sampled at $2.4\,\text{Msps}$. Its parameters are $A(t)=2$, $\theta_{\mathrm{Tx}}-\theta_{\mathrm{Rx}} = 0$, and $S=7$. Thus, the chirp time $\frac{2^S}{W}$ is $1.024\,\text{ms}$. To generate the spectrogram, we apply the short-time fast Fourier transform (FFT) with $2^S$-point Kaiser window and 16-point overlap between two neighbor windows. Thus, the spectrogram consists of 20 power spectral densities over the chirp time of $1.024\,\text{ms}$.

\begin{figure}
  \centering
  \includegraphics[width=.22\textwidth]{./Figures/cI_preamble_zero_phase}
  \hspace{1em}
  \includegraphics[width=.22\textwidth]{./Figures/cspec2}
  \caption{$I$ data ($\theta_{\mathrm{Tx}}$=$\theta_{\mathrm{Rx}}$) and spectrogram of a preamble chirp.}
  \label{fig:up-chirp}
\end{figure}

\subsubsection{Preamble onset time detection}
\label{subsubsec:preamble-onset}

\begin{figure}
  \centering
  \begin{minipage}[t]{.22\textwidth}
    \includegraphics[width=\textwidth]{./Figures/cI_preamble_diff_phases}
    \caption{$I$ data of a preamble chirp with $\theta_{\mathrm{Tx}} - \theta_{\mathrm{Rx}}=0$ (the red curve) or $\theta_{\mathrm{Tx}} - \theta_{\mathrm{Rx}}=\pi$ (the blue curve).}
    \label{fig:preamble_I_data_all}
  \end{minipage}
  \hspace{.01\textwidth}
  \begin{minipage}[t]{.22\textwidth}
    \includegraphics[width=\textwidth]{./Figures/cI_raw_signal2}
    \caption{Actual $I$ data of a preamble chirp. The time shift of the dip center is caused by FB.}
    \label{fig:I_signal}
  \end{minipage}
\end{figure}

Detecting the onset time of the preamble is non-trivial.
Matched filter is a widely adopted symbol detection technique. As a coherent detection technique, the matched filter requires that the receiver is phase-locked to the transmitter (i.e., $\theta_{\mathrm{Tx}}=\theta_{\mathrm{Rx}}$) to achieve the best symbol detection accuracy. However, as LoRa adopts time-varying frequency, it is difficult for the SDR receiver to estimate the transmitter's phase $\theta_{\mathrm{Tx}}$.
As a result, the phase difference $\theta_{\mathrm{Tx}}-\theta_{\mathrm{Rx}}$, which is a critical factor affecting the shape of $I(t)$ and $Q(t)$, will be random. Fig.~\ref{fig:preamble_I_data_all} shows the ideal $I(t)$ traces of the preamble chirp when the phase difference is $0$ and $\pi$. The waveform shapes are different. Thus, we cannot define a template shape required by the matched filter. Moreover, as analyzed in \sect\ref{sec:fingerprint}, the FB of the LoRa transmitter will significantly alter the shapes of the $I$ and $Q$ signals. Fig.~\ref{fig:I_signal} shows an actual $I$ trace captured by the SDR receiver. The time shift of the dip center is caused by FB.
Thus, due to the random phase difference and the LoRa transceiver's FB, the matched filter is not promising.

\begin{figure}
  \subfigure[ENV detector]
  {
    \includegraphics[width=.22\textwidth]{./Figures/craw_signal}
    \label{fig:I_envelope}
  }
  \subfigure[AIC detector]
  {
    \includegraphics[width=.22\textwidth]{./Figures/cARAIC_detector}
    \label{fig:I_araic}
  }
  \caption{Detecting onset time of first preamble chirp (S=12).}
  \label{fig:onset}
\end{figure}

For $\mathsf{LoRaTS}$, we consider two parameter-less detectors:

\noindent {\bf Envelope (ENV) detector:} First, we apply the Hilbert transform to extract the amplitude envelope of the $I$ or $Q$ signal. Then, the sample with the largest ratio between its envelope amplitude and the previous sample's envelope amplitude is yielded as the preamble onset. Fig.~\ref{fig:I_envelope} shows the extracted amplitude envelope and the detected onset time represented by the vertical line.

\noindent {\bf AIC detector:} The autoregressive Akaike Information Criterion (AIC) algorithm \cite{sleeman1999robust} can detect the onset time of an oscillatory signal. It works as follows. For each point of the signal as an onset time candidate, two autoregressive models are constructed for the signal segments before and after the onset time candidate. The candidate that gives the largest dissimilarity between the two autoregressive models is yielded as the final result. From Fig.~\ref{fig:I_araic}, AIC can detect the onset time from the signal with a smooth start. From the results in \cite{sleeman1999robust}, AIC's detection results have a bias of 4 samples. With a sampling rate of $2.4\,\text{MHz}$, the bias is $\mathbb{E}[\epsilon]=\frac{4}{2.4\,\text{Msps}} = 1.67\,\mu\text{s}$ only, where $\epsilon$ represents onset time detection error.

\subsubsection{Evaluation of ENV and AIC}
\label{subsec:accuracy-evaluation}

We conduct a set of experiments to evaluate the performance of the ENV and AIC detectors. As AIC is nearly unbiased \cite{sleeman1999robust}, we primarily assess the root-mean-square deviation (RMSD) which characterizes the consistency of the detection results. Due to the difficulty in obtaining the ground truth of the preamble arrival time, we indirectly estimate the RMSD as follows. We place two $\mathsf{LoRaTS}$ nodes $A$ and $B$ close to each other such that signal propagation time is near-zero. Node $A$ initiates a round-trip communication; each of them detects the onset times for both its transmitted and received signals, generating totally four onset times. Note that a $\mathsf{LoRaTS}$ node's SDR receiver can also capture the signal transmitted by the node's LoRa radio and detect the onset time. Denote by $\Delta$ the measured round-trip time based on the detected onset times; denote by $\epsilon_{X}^{Tx}$ and $\epsilon_{X}^{Rx}$ the node $X$'s unknown onset time detection errors for its transmitted and received signals. We can derive $\Delta = \epsilon_{A}^{Rx} - \epsilon_{A}^{Tx} + \epsilon_{B}^{Rx} - \epsilon_{B}^{Tx}$ and $\mathrm{RMSD}(\epsilon) = \frac{1}{2} \mathrm{RMSD}(\Delta)$ if the errors are independent and identically distributed. Measurements show that $\mathrm{RMSD}(\epsilon)$ is $1.21\,\mu\text{s}$ and $0.33\,\mu\text{s}$ for ENV and AIC, respectively. Thus, AIC achieves more consistent detection results. Then, we evaluate the impact of random noises on AIC's $\mathrm{RMSD}(\epsilon)$. We artificially add zero-mean Gaussian noises to the collected high-SNR $I$ and $Q$ traces. Then, we apply AIC on the noise-added traces to detect the preamble onset time. Fig.~\ref{fig:ar-aic-snr} shows the results. Note that the SNR range in Fig.~\ref{fig:ar-aic-snr} can cover realistic SNRs, e.g., $13\,\text{dB}$ to $-1\,\text{dB}$ in a multistory building (cf.~\sect\ref{sec:eval}). From Fig.~\ref{fig:ar-aic-snr}, the AIC's $\mathrm{RMSD}(\epsilon)$ is less than $5\,\mu\text{s}$ when the SNR is down to $-20\,\text{dB}$. Thus, AIC achieves robust onset time detection in the presence of strong noises. The rest of this paper uses AIC.

%%% Local Variables:
%%% mode: latex
%%% TeX-master: "secure-ts"
%%% End:

==> Makefile <==
DOC=secure-ts

all:
	pdflatex $(DOC).tex
	bibtex $(DOC)
	pdflatex $(DOC).tex
	pdflatex $(DOC).tex

clean:
	rm -f *.blg *.bbl *.aux *.log *.pdf *.synctex.gz* *.fls *.fdb_latexmk

cleanpdf:
	rm -f *.pdf

dvi:
	if [ ! -f dvimode ] ; \
	then \
		echo "Entering dvimode" ; \
		echo "" > dvimode ; \
		sed -i '/\RequirePackage\[libertine\]{newtxmath}/c\\\RequirePackage\[italic\]{mathastext}' acmart.cls; \
		sed -i '/\RequirePackage\[prologue\]{xcolor}/c\\\RequirePackage{xcolor}' acmart.cls; \
	fi;
	latex -src-specials -halt-on-error $(DOC)
	#latex -src-specials -halt-on-error -jobname=lora-sync-techreport $(DOC)

bib:
	bibtex $(DOC)

pdf:
	if [ -f dvimode ] ; \
	then \
		echo "Exiting dvimode" ; \
		rm -f dvimode ; \
		sed -i '/\RequirePackage\[italic\]{mathastext}/c\\\RequirePackage\[libertine\]{newtxmath}' acmart.cls; \
		sed -i '/\RequirePackage{xcolor}/c\\\RequirePackage\[prologue\]{xcolor}' acmart.cls; \
	fi;
	latex $(DOC)
	dvips $(DOC).dvi 
	ps2pdf $(DOC).ps

upload:
	unison ../ICDCS20_submission ../../Secure-TS/ICDCS20_submission

# drop:
	# unison ~/research/LoRa-sync/writeup5 ~/Dropbox/Secure-TS/ICDCS20_submission

spell:
	rm -f $(DOC).out
	lualatex $(DOC)
	lt --api -l en-US $(DOC).spell.txt > $(DOC).spell.xml
	lualatex $(DOC)

techreport:
	latex -jobname=lora-sync-techreport $(DOC)
	bibtex lora-sync-techreport
	latex -jobname=lora-sync-techreport $(DOC)
	latex -jobname=lora-sync-techreport $(DOC)
	dvips lora-sync-techreport.dvi
	ps2pdf lora-sync-techreport.ps

icdcs:
	pdflatex -jobname=icdcs-submission $(DOC).tex
	bibtex icdcs-submission
	pdflatex -jobname=icdcs-submission $(DOC).tex
	pdflatex -jobname=icdcs-submission $(DOC).tex

full-text:
	pdflatex $(DOC).tex
	bibtex $(DOC)
	pdflatex $(DOC).tex
	pdflatex $(DOC).tex
